Enhancing Tool Retrieval with Iterative Feedback from Large Language Models

Tool learning aims to enhance and expand large language models' (LLMs) capabilities with external tools, which has gained significant attention recently. Current methods have shown that LLMs can effectively handle a certain amount of tools through in-context learning or fine-tuning. However, in real-world scenarios, the number of tools is typically extensive and irregularly updated, emphasizing the necessity for a dedicated tool retrieval component. Tool retrieval is nontrivial due to the following challenges: 1) complex user instructions and tool descriptions; 2) misalignment between tool retrieval and tool usage models. To address the above issues, we propose to enhance tool retrieval with iterative feedback from the large language model. Specifically, we prompt the tool usage model, i.e., the LLM, to provide feedback for the tool retriever model in multi-round, which could progressively improve the tool retriever's understanding of instructions and tools and reduce the gap between the two standalone components. We build a unified and comprehensive benchmark to evaluate tool retrieval models. The extensive experiments indicate that our proposed approach achieves advanced performance in both in-domain evaluation and out-of-domain evaluation.

==> tabs/case_study.tex <==
\begin{table*}[t]
\centering
\small
\resizebox{\linewidth}{!}{
\begin{tabularx}{\textwidth}{l|l|l|l|l}
\toprule
&
\multicolumn{1}{c|}{\textbf{Iteration 0}} &  
% \multicolumn{2}{c|}{\textbf{Iteration 1}} &
\multicolumn{1}{c|}{\textbf{Iteration 1}} &
\multicolumn{1}{c|}{\textbf{Iteration 2}} &
\multicolumn{1}{c}{\textbf{Iteration 3}} \\ \midrule
% {\textbf{Iteration 0}} & 
% {\textbf{Iteration 1}} & 
% {\textbf{Iteration 2}} & 
% {\textbf{Iteration 3}} \\ \midrule
% \multicolumn{3}{c}{\textbf{{All}}} \\ 
% \cmidrule(lr){2-13}
% \multicolumn{1}{Y|}
{Refined Instruction} & 
\multicolumn{1}{X|}{Please assist me in finding the latest versions of Bash. Additionally, I require a new datacenter proxy with whitelisted IPs. Can you provide the details of the proxy, including the host, port, and expiration time? Also, I would like to check the current service status of the residential proxies.} &
\multicolumn{1}{X|}{Please assist me in finding the latest versions of Bash. Additionally, I require a new datacenter proxy with whitelisted IPs. Can you provide the details of the proxy, including the host, port, and expiration time? Also, I would like to check the current service status of the residential proxies and obtain {information} about the \colorbox{yellow}{total number} of available residential proxies grouped by country.} &
\multicolumn{1}{X|}{Please assist me in finding the latest versions of Bash. Additionally, I require a new datacenter proxy with whitelisted IPs. Can you provide the details of the proxy, including the host, port, and expiration time? Also, please provide the current service status of the residential proxies, including \colorbox[rgb]{0.95,0.5,0.5}{\sout{information about}} the total number of proxies available and grouped by country.} &
\multicolumn{1}{X}{N/A} \\ \midrule
% N/A \\ \midrule

% \makecell[l]{...\\...}


\multirow{3}{*}{\makecell[l]{Retrieved Candidate \\ Tools}} & 
% \multirow{3}{*}{\multicolumn{1}{X}{Retrieved Candidate Tools}} & 
% \multicolumn{1}{p{0.2\linewidth}}
\multicolumn{1}{X|}{Tools, Ephemeral Proxies, Obtain a new datacenter proxy...
% , The connection proxy details are `proxy.host` and `proxy.port` from the response fields. 
% The proxy will allow connections from the same source IP as the one making this API call. 
% Make use of the `whitelist\_ip` parameter to allow an additional ip. 
% Countries can be selected by using the `countries` parameter, otherwise the country is randomly selected. A list of countries is available on *Service Status* endpoint. The proxy is available for 30 mins...
} &
\multicolumn{1}{X|}{Tools, Ephemeral Proxies, Obtain a new datacenter proxy...} &
\multicolumn{1}{X|}{Tools, Ephemeral Proxies, Obtain a new datacenter proxy...} &
\multicolumn{1}{X}{Tools, Ephemeral Proxies, Obtain a new datacenter proxy...} \\ \cmidrule(lr){2-5}
% \cmidrule(l{5em}r{5em}){1-2}
&
\multicolumn{1}{X|}{
Tools, Ephemeral Proxies, Extend expiration time of a datacenter proxy...
% , By calling this endpoint the expiration time of an already allocated proxy will be extended by 30 mins.
% Successive calls will keep incrementing the expiration time, up to a maximum of 24 hours.
} &
\multicolumn{1}{X|}{Tools, Ephemeral Proxies, Check residential proxies service status...
% , It returns the current status of the service, 
including the \colorbox{yellow}{total number} of residential proxies...
% available and grouped by country.
} &
\multicolumn{1}{X|}{Tools, Ephemeral Proxies, Check residential proxies service status...
% , It returns the current status of the service, 
including the total number of residential proxies...
% available and grouped by country.
} &
\multicolumn{1}{X}{Tools, Ephemeral Proxies, Check residential proxies service status...
% , It returns the current status of the service, 
including the total number of residential proxies...
% available and grouped by country.
} \\ \cmidrule(lr){2-5}
% & 

% Tools, Proxy Checker, Retrieve Proxy Information...
% , For retrieving a proxy test result, you should make a request to this endpoint...


% Tools, Ephemeral Proxies, Extend expiration time of a datacenter proxy, By calling this endpoint the expiration time of an already allocated proxy will be extended by 30 mins.\nSuccessive calls will keep incrementing the expiration time, up to a maximum of 24 hours.

% Data, Proxy-Spider Proxies, /proxies.example.json, This is a free sample of ten proxies. Sign up and receive the full list.

% Tools, Proxy Checker, Retrieve Proxy Information, For retrieving a proxy test result, you should make a request to this endpoint...
% \\
&
% \colorbox[rgb]{0.95,0.5,0.5}{
\multicolumn{1}{X|}{
Data, Proxy-Spider Proxies, /proxies.example.json...
% }
% , This is a free sample of ten proxies. Sign up and receive the full list...
} &
\multicolumn{1}{X|}{Tools, Proxy Checker, Retrieve Proxy \colorbox[rgb]{0.95,0.5,0.5}{Information}...
% , For retrieving a proxy test result, you should make a request to this endpoint...
} &
\multicolumn{1}{X|}{Tools, Bash Code Compiler, Bash Versions...} &
\multicolumn{1}{X}{Tools, Bash Code Compiler, Bash Versions...} \\ \midrule

% \makecell[c]{% }


\multirow{3}{*}{Ground-truth Tools} &
\multicolumn{4}{p{0.8\linewidth}}{
% \shortstack{
Tools, Ephemeral Proxies, Check residential proxies service status, 
It returns the current status of the service, 
including the total number of residential proxies available and grouped by country...
} \\
& 
\multicolumn{4}{p{0.8\linewidth}}{
Tools, Ephemeral Proxies, Obtain a new datacenter proxy...
} \\
& 
\multicolumn{4}{p{0.8\linewidth}}{
Tools, Bash Code Compiler, Bash Versions, Bash Versions...
} \\
\bottomrule
\end{tabularx}}
\caption{Case study.} 
\label{case_study}
\end{table*}
